Regularized Training of Intermediate Layers for Generative Models for Inverse Problems

Generative Adversarial Networks (GANs) have been shown to be powerful and flexible priors when solving inverse problems. One challenge of using them is overcoming representation error, the fundamental limitation of the network in representing any particular signal. Recently, multiple proposed inversion algorithms reduce representation error by optimizing over intermediate layer representations. These methods are typically applied to generative models that were trained agnostic of the downstream inversion algorithm. In our work, we introduce a principle that if a generative model is intended for inversion using an algorithm based on optimization of intermediate layers, it should be trained in a way that regularizes those intermediate layers. We instantiate this principle for two notable recent inversion algorithms: Intermediate Layer Optimization and the Multi-Code GAN prior. For both of these inversion algorithms, we introduce a new regularized GAN training algorithm and demonstrate that the learned generative model results in lower reconstruction errors across a wide range of under sampling ratios when solving compressed sensing, inpainting, and super-resolution problems.

==> sections/appx-theory.tex <==
\newpage
\section{Proof}

\begin{proof}[Proof of Lemma \ref{lemma:training}]
Notice that for any $W_1 \in \R^{n_d \times n_1}$
\[
    \begin{aligned}
    \E_{z_0, z_1} [\| \Wstar_1 (\Wstar_0 z_0 + z_1) - W_1 \Wstar_0 z_0  \|_2^2]
    &= \E_{z_0} [\| (\Wstar_1 - W_1) \Wstar_0 z_0 \|_2^2] + \E_{z_1} [\| \Wstar_1 z_1 \|_2^2]\\
    &= \| (\Wstar_1 - W_1 )\Wstar_0 \|_F^2 + \|\Wstar_1\|^2_F,
    \end{aligned}
\]
where the first equality used independence of $z_0$ and $z_1$ and the second used the fact that $\E_{z \sim \mathcal{N}(0,I_n)}\| M z\|_2^2 = \|M\|_F^2$ for any matrix $M \in \R^{m \times n}$.
The solutions of \eqref{eq:W11} are then solutions of 
\begin{equation}\label{eq:calF}
     \min_{W_1 \in \R^{n_1 \times n_0}} \| \mathcal{L}(\Wstar_1) - \mathcal{L}(W_1)\|_F^2
\end{equation}
where $\mathcal{L}: \R^{n_d \times n_1} \to \R^{n_1 \times n_0}$ is the linear operator given by $\mathcal{L}: W_1 \mapsto W_1 \Wstar_0$. Since  $n_1 > n_0$, this operator is singular and there are infinite solutions of \eqref{eq:calF}, all of which satisfy $\mathcal{L}(\Wstar_1) = \mathcal{L}(W_1)$, i.e. the thesis.


Regarding \eqref{eq:W12}, observe instead that for any $W_1 \in \R^{n_d \times n_1}$ 
\[
\begin{aligned}
\E_{z_0, z_1} [\| \Wstar_1 (\Wstar_0 z_0 + z_1) - W_1 (\Wstar_0 z_0 + z_1)  \|_2^2]
&= \| (\Wstar_1 - W_1) \Wstar_0 \|_F^2 + \|\Wstar_1 - W_1\|^2_F.
\end{aligned}
\]
This shows $W_1 = \Wstar_1 $ is the unique minimizer of \eqref{eq:W12}.
\end{proof}


Before analyzing the solution of compressed sensing with the trained generative models, we observe the following fact on the minimum norm solution of \eqref{eq:W11}. 

\begin{lemma}\label{eq:minNorm}
Let $W_1^{0}$ be the minimum Frobenius norm solution of \eqref{eq:W11}. Then $W_1^{0} = \Wstar_1 \Wstar_0 (\Wstar_0)^\dagger$ where $(\Wstar_0)^\dagger$ is the pseudoinverse of $\Wstar_0$.
\end{lemma}
\begin{proof}
    Notice that $\mathcal{L}(\Wstar_1) = \mathcal{L}(W_1^{(1)})$, where $\mathcal{L}$ is defined in the proof of Lemma \eqref{lemma:training}.  
    We next show that $W_1^{0}$ is orthogonal to the null space of $\mathcal{L}$, which implies the thesis. 
    
    Let $W_1 \in \R^{n_d \times n_1}$ be such that $\mathcal{L}(W_1) = W_1 \Wstar_0 = 0$. Then we have
    \[
    \begin{aligned}
        \langle W_1^{0}, W_1\rangle_F &= tr((W_1^{0})^T W_1) \\ 
        &= tr(W_1 (\Wstar_0 (\Wstar_0)^\dagger)^T (\Wstar_1)^T ) \\
        &= tr(W_1 \Wstar_0 (\Wstar_0)^\dagger (\Wstar_1)^T ) \\ 
        &= 0,
    \end{aligned}
    \]
    where third equality uses the fact that $\Wstar_0 (\Wstar_0)^\dagger$ is symmetric and the fourth one the assumption on $W_1$.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:CS}]
\smallskip${}$

- {Proof of \eqref{eq:ERR1}}.
Notice that by the previous lemma $W_1^{0} = \Wstar_1 \Wstar_0 (\Wstar_0)^\dagger = \Wstar_1 \mathcal{P}_{\Wstar_0}$  where $\mathcal{P}_{\Wstar_0}$ is the orthogonal projector onto the range of $\Wstar_0$. Moreover, with probability 1, $(A \Wstar_1 \Wstar_0 )$ is full rank.
It follows then, that $(z_0^{(0)}, z_1^{(0)})$ is given by
\[
\begin{aligned}
    z_0^{(0)} &= \argmin_{z_0 \in \R^{n_0}} \| y - A \Wstar_1 \Wstar_0 z_0 \|_2^2, \\
    z_1^{(0)} &= \argmin_{z_1 \in \R^{n_1}} \| y - A \Wstar_1 ( \Wstar_0 z_0^{(0)} + \mathcal{P}_{\Wstar_0} z_1 )\|_2^2. 
\end{aligned} 
\]
In particular the minimum norm solution $z_1^{(0)}$ will satisfies $(I - \mathcal{P}_{\Wstar_0})z_1^{(0)} = 0$. We have therefore $G^{(1)}(z_0^{(0)}, z_1^{(0)}) =  \Wstar_1 (\Wstar_0 \zstar_0 +  \Wstar_0 \mathcal{M}_1^{(0)} \zstar_1)$ where $\mathcal{M}_1^{(0)} = (A \Wstar_1 \Wstar_0 )^\dagger \Wstar_1$. 

The reconstruction error is then given by
    \[
    \begin{aligned}
        \E_{\zstar_0, \zstar_1} \| G^\star(\zstar_0, \zstar_1) -  G^{0}(z_0^{(0)}, z_1^{(0)}) \|_2^2 
        &=   \| \Wstar_1   - \Wstar_1 \Wstar_0 \mathcal{M}_1^{0} \|_F^2 \\
        &\geq \min_{\mathcal{M}_1 \in \R^{n_0 \times n_1} } \| \Wstar_1   - \Wstar_1 \Wstar_0 \mathcal{M}_1 \|_F^2\\
        &= \|\big(I_{n_d} - \mathcal{P}_{\Wstar_1 \Wstar_0} \big) \Wstar_1 \|_F^2
    \end{aligned}
    \] 
    where the first equality follows from the properties of the normal distribution. Regarding then the minimization problem $\min_{\mathcal{M}_1 \in \R^{n_0 \times n_1} } \| \Wstar_1   - \Wstar_1 \Wstar_0 \mathcal{M}_1 \|_F^2$, notice that this is convex and the critical points satisfy
    \[
         (\Wstar_1 \Wstar_0)^T  \Wstar_1  = (\Wstar_1 \Wstar_0)^T (\Wstar_1 \Wstar_0) \mathcal{M}_1
    \]
    Using the fact that $\Wstar_1 \Wstar_0$ is full rank, the unique solution is found to be $[ (\Wstar_1 \Wstar_0)^T (\Wstar_1 \Wstar_0) ]^{-1}(\Wstar_1 \Wstar_0)^T  \Wstar_1 $, which gives the last equality. 
    \smallskip
    
    Note now that $\mathcal{P}_{\Wstar_1 \Wstar_0}$ is the projector onto the range of $\Wstar_1 \Wstar_0$ and $\Wstar_1$ is full rank. Thus
    \[
        \|\big(I_{n_d} - \mathcal{P}_{\Wstar_1 \Wstar_0} \big) \Wstar_1 \|_F^2
        \geq \|\big(I_{n_d} - \mathcal{P}_{\Wstar_1 \Wstar_0} \big) \Wstar_1 \|_2^2
        = \max_{h \in \text{range}(\Wstar_0)^\perp}\|\big(I_{n_d} - \mathcal{P}_{\Wstar_1 \Wstar_0} \big) \Wstar_1 h\|_2^2 > 0.
    \]
    \medskip
    
    - \textit{Proof of \eqref{eq:ERR2}}
    Notice again that with probability 1, $A \Wstar_1 \Wstar_0$ and $A \Wstar_1$ have full rank. Moreover $G^{1}(z_0^{(1)}, z_1^{(1)}) =  \Wstar_1 (\Wstar_0 z_0^{(1)} +  z_1^{(1)})$ where 
    \[
    \begin{aligned}
        z_0^{(2)} &= \argmin_{z_0 \in \R^{n_0}} \| y - A W_1^{(1)} \Wstar_0 z_0 \|_2^2, \\
        z_1^{(1)} &= \argmin_{z_1 \in \R^{n_1}} \| y - A W_1^{(1)}( \Wstar_0 z_0^{(1)} + z_1 )\|_2^2. \\
    \end{aligned} 
    \]
    It is then easy to see that
    \[
        \begin{aligned}
            z_0^{(1)} &= \zstar_0 + (A \Wstar_1 \Wstar_0 )^\dagger A \Wstar_1 \zstar_1 \\
            z_1^{(1)} &= \zstar_1 - \Wstar_0 (A \Wstar_1 \Wstar_0 )^\dagger A \Wstar_1 \zstar_1 
        \end{aligned}
    \]
    where $(A \Wstar_1 \Wstar_0 )^\dagger$ denotes the pseudoinverse of $(A \Wstar_1 \Wstar_0 )$. It then follows that $\Wstar_1 (\Wstar_0 z_0^{(1)} +  z_1^{(1)}) =\Wstar_1 (\Wstar_0 z_0^\star +  z_1^\star) = x^\star$, which implies the thesis.
\end{proof}

==> sections/sec-rtil.tex <==
\section{RTIL}


\begin{figure}[h!]
	\begin{center}
	\includegraphics[width=1.0\linewidth]{figs/mGANprior/cs_mgan_5_ssim.png}
	\end{center}
	\caption{Comparison between mGANprior-RTIL (ours) and mGAN for compressed sensing  for 5\% of measurements. }
	\label{mGANprior_cs}
\end{figure}


In this section, we present how the principle of   Regularized Training of Intermediate Layers (RTIL) inspires training algorithms for GANs that are intended for inversion by Intermediate Layer Optimization (Section \ref{subsec:RTIL-ILO}) and  mGANprior (Section \ref{subsec:RTIL-mGANprior}).
  
%We show that intermediate layers can be effectively regularized by training multiple generative models at the same time, an underlying vanilla model and one or more variations where noise is injected at one or more intermediate layers, with parameter sharing across each model.
%We next overview training and inversion based on our RTIL principle for generic intermediate optimization inversion algorithmic. In .  


We consider the case of a practitioner having chosen, after some initial exploration, a base generative network $G_{\theta}^{0}$ for use as prior in solving inverse problems. For simplicity in this section we will consider   $G_{\theta}^{0} = g_1 \circ g_0$ where $g_0 : \R^{n_0} \to \R^{n_1}$ and $g_1: \R^{n_1} \to \R^{n_d}$. 
The input latent vectors $z_0$ of the network $G_{\theta}^{0}$ are sampled from $p_{z_{0}}$ (e.g. $p_{z_0} \sim \mathcal{N}(0,\I_{n_{0}})$) and $\theta$ is the set of trainable weights. 
%For brevity, we write $G_{\theta}^{0} (p_{z_{0}})$ as the generative model. 

We assume, furthermore, that the practitioner has selected an inversion algorithm that optimizes over the latent variable $z_0$ and the intermediate layer between $g_0$ and $g_1$ of $G_\theta^{0}$.  Optimizing over the intermediate layer corresponds to introducing a free variable $z_1$ between $g_0$ and $g_1$  (Figure \ref{fig:rtil_general} left).

The RTIL principle states that if one intends to solve inverse problems by means of intermediate layer optimization algorithms, then 
\textit{intermediate layers optimized over during inversion should be regularized during training}.

This principle can be used to design a new training algorithm in the following manner. We identify the additional free variable, $z_1$, used for optimization over the intermediate layer, consider it as a latent variable of the generative model, and provide it with a simple distribution $p_{z_{1}}$.  
%We consider a model where $z_1$ is combined with the output of $g_0$ before it is passed into $g_1$.  
This results in a generative model $G_{\theta} : \R^{n_0 \times n_1} \to \R^{n_d}$, such that $G_\theta (z_0 , z_1) = g_1 (z_1 + g_0(z_0))$

.  This generative model reduces to the base generative model if $z_1$ is suitably chosen, for example if $z_1=0.$  For ease of exposition, we write this as 
$G_{\theta} (p_{z_{0}},0) \equiv G_{\theta}^{0} (p_{z_{0}})$. See Figure~\ref{fig:rtil_general}. 
%, and therefore the intermediate layer, is regularized by training a new generative network based on the inversion method chosen. The latter is in particular used to inform the choice of the latent distribution $p_{z_{1}}$ from which the latent variables $z_1$ are sampled during training. 

The introduction of the latent variable $z_1$ explicitly increases the dimensionality of the latent space. In practice, training latent variable models with high-dimensional latent spaces can be challenging and require careful regularization 
%to fit the data distribution 
~\citep{athar2018latent}. We address this difficulty by concurrently training the family of generative models  $\{G_{\theta} (p_{z_{0}},0),G_{\theta}(p_{z_{0}},p_{z_{1}}) \}$ that shares trainable weights $\theta$ (Figure \ref{fig:rtil_general} right).

We train $G_{\theta}$ via the following minimax formulation~\citep{NIPS2014_5ca3e9b1}
\begin{align*}
%\label{eq:min-max}
\min_{G_{\theta}} \max_{D_{\Theta}} V(D_{\Theta},G_{\theta}) 
&=  \E_{ x \sim p_{x}} [ \log D_\Theta(x) ] \notag \\ \ \ \ \ \ \ \ \  + \E_{\substack{ z_{0} \sim p_{z_{0}} \\  z_{1} \sim p_{z_{1}} }}   
 &\big[ \frac{1}{2}  \log(1-D_\Theta(G_{\theta}(p_{z_{0}},0)) \\&+ \frac{1}{2}\log(1-D_\Theta(G_{\theta}(p_{z_{0}},p_{z_{1}})) \big],\notag
\end{align*}
where $D_\Theta: \R^{n_d} \to \R$ is the discriminative network.  This method could be extended to alternative GAN and non-GAN formulations ~\citep{arjovsky2017wasserstein,gulrajani2017improved}. {\color{red} Add citation to Generative Latent Optimization. }
%attempts to distinguish between the generated samples from $G_{\theta}(p_{z_{0}},0)$ and $G_{\theta}(p_{z_{0}},p_{z_{1}})$, and the training data. 

%Note that because of the weight sharing, the computational cost of training the family of generative networks remains essentially the same as the original base network $G_{\theta}^{0}$.

Once $G_{\theta}$ is trained, a practitioner  would solve an inverse problem with forward operator $\mathcal{A}$ by solving
%would then use $G_{\theta}(p_{z_{0}},p_{z_{1}})$, the network with the largest number of latent variables and more expressivity, for solving inverse problems.
%Specifically, for an inverse problem with forward a, the originally chosen inversion method  is applied
%on the following minimization problem
\begin{equation*}%\label{eq:min_G2}
\hat{{z}}_{0}, \hat{{z}}_{1} = \underset{z_{0}, z_1}{\argmin} \hspace{2mm} \|y_{0}- \mathcal{A}(G_\theta(z_{0}, z_{1})) \|,
\end{equation*}
using the selected optimization algorithm, resulting in $G_\theta(\hat{z}_{0}, \hat{z}_{1})$ as the estimate of the signal.

In this section, we considered the case where only one intermediate layer was optimized.  The proposed method can directly extend to the case where multiple layers are optimized.


% We conclude noticing that the existing inversion methods that optimize over $z_0, z_1$ and use $G^{0}$, violates the generative prior assumption when solving inverse problems, as $z_1$ was not explicitly regularized during training. In contrast, our proposed RTIL guarantees that during the inversion phase  $G_\theta$ preserves the  generative prior assumption, and as shown in the experiments, this leads to improved reconstruction performances.

\begin{comment}
\begin{figure}
\def\svgwidth{\linewidth}
\import{figs/}{inversion-rtil.pdf_tex}
%\includegraphics[width=1.0\linewidth]{figs/RTIL_pic_horiz_v3.png}
\caption{Visual representation of the RTIL principle.  An  inversion method that optimizes over intermediate layers informs the training of a family of generative networks adapted to that inversion method.}
\label{fig:rtil_general}
\end{figure}
\end{comment}

\begin{figure}
\includegraphics[width=1.\linewidth,height=4cm]{figs/inversion-rtil.pdf}
\caption{Visual representation of the RTIL principle.  An  inversion method that optimizes over intermediate layers informs the training of a family of generative networks adapted to that inversion method.}
\label{fig:rtil_general}
\end{figure}

We will next describing the details of the application of RTIL in the case of Intermediate Layer Optimization and the Multi-Code GAN Prior.   


\subsection{RTIL for ILO}\label{subsec:RTIL-ILO}


\begin{figure*}[h]
%\def\svgwidth{\linewidth}
\includegraphics[width=1.\linewidth]{figs/ILO/rtil-ilo.pdf}
\caption{ The left side portrays ILO, and the right side demonstrates how this inspire the training of a family of generative models with ILO-RTIL with parameters sharing.}
%\caption{}
\label{fig:rtil_ILO}
\end{figure*}


In the case of Intermediate Layer Optimization (ILO), we now present how to use RTIL to design a GAN training algorithm.  Consider the base generative network $G(z_0) =g_{1} ( g_{0} (z_0))$, to be used for inversion with Intermediate Layer Optimization. ILO (Algorithm \ref{alg:ILO}) extends the range of the network by optimizing  $g_{1}(z_{1} + g_{0} ({z}_{0}) )$ over latent variables $z_0$ and $z_1$. Consequently, we consider an extended generative model
\begin{align*}
    G_\theta(z_0, z_1) &= g_{1}(z_{1} + g_{0} ({z}_{0}) )\\
    z_0 &\sim \mathcal{N}(0, I_{n_0})\\
    z_1 &\sim \mathcal{N}(0, I_{n_1})
\end{align*}
simultaneously training a family of generative models $\{G_{\theta} (p_{z_{0}},0),G_{\theta}(p_{z_{0}},p_{z_{1}}) \}$, where the first model of the family is given by $G_{\theta} (p_{z_{0}},0)=g_{1}(g_{0}(z_{0}))$ and the second model is given by $G_{\theta}(p_{z_{0}},p_{z_{1}}) = g_{1}(z_{1} + g_{0} ({z}_{0}) )$. Note $z_0 \sim p_{z_0}$ and  $z_1 \sim p_{z_1}$ where
Figure \ref{fig:rtil_ILO} depicts this process.


%Analyzing the Intermediate Layer Optimization method is evident that this consists in optimizing over $z_0$ and an additional latent variable $z_1$ which  simply perturbs the output of the first layer (Figure \ref{fig:rtil_ILO} right).  


%Applying, therefore,  
%RTIL we are led to then train, via the min-max formulation \eqref{eq:min-max}, the family of generative networks with shared weights $G_{\theta} = \{G_{\theta} (p_{z_{0}},0),G_{\theta}(p_{z_{0}},p_{z_{1}}) \}$  (Figure \ref{fig:rtil_ILO} right). Given the interpretation of $z_1$ as a perturbation off the range of $g_0$, it is natural to consider $p_{z_1} \sim \mathcal{N}(0, \sigma^2 I_{n_1})$ where $\sigma$ is a tunable standard deviation.

%After training, ILO is applied to the network $G_{\theta}(p_{z_{0}},p_{z_{1}})$ which has learned, during training, regularized and semantically meaningful perturbations $z_1$.   


%Note that, this method can be extended to deeper networks and a larger family of generative models, by simply increasing the number of intermediate layers chosen. \cut In our experiments, we trained multiple models including latent variables up to the intermediate layer having input dimension larger than dimension of the target data distribution.

%During inversion when applying RTIL-ILO as a prior, the training procedure is consistent with the ILO optimization algorithm solved downstream because the intermediate layers are regularized by the distributions induced during training. Searching over the extended set  when optimizing  RTIL-ILO will have the expressivity to learn meaningfully distribution to best fit the measurements. From the perspective the interpretation is analogous where optimizing over each intermediate layer that initialized from the previous the learned distribution in optimization will perturb when searching over the set, so during training to increase performance regularize that set.  

\subsection{RTIL for mGANprior}\label{subsec:RTIL-mGANprior}

\begin{comment}
\begin{figure*}[h]
\def\svgwidth{\linewidth}
\import{figs/mGANprior}{mgan-rtil.pdf_tex}
\caption{The left side portray vanilla training for mGANprior, and the right side demonstrates RTIL. For  mGANprior-RTIL this example with $N = 2$ latent codes, where the top model trains a vanilla model analogous to model on the left, then parameter shares with the model below to induce a distribution in the intermediate layers. }
\label{fig:rtil_mgan}
\end{figure*}
\end{comment}

In the case of Multi-Code GAN Prior method, we now present how to use RTIL to design a GAN training algorithm.  Consider the base generative network $g_{1} \circ g_{0}$ 
to be used for inversion with the Multi-Code GAN Prior method.
The mGANprior Algorithm (Algorithm \ref{alg:mGAN}) extends the range of the network by optimizing  $g_{1}(\sum_{k=1}^{N}g_{0}({z}_{0}^{k}) \odot {\alpha}^{k})$ over latent variables $z_0$ and $z_1$. Consequently, we consider simultaneously training a family of generative models $ \{G_{\theta}(p_{z_{0}},0), G_\theta(p_{z_0^1}, \dots, p_{z_0^N}, p_{\alpha^1}, \dots, p_{\alpha^N }\}$, where the first model of the family is given by $G_{\theta} (p_{z_{0}},0)=g_{1}(g_{0}(z_{0}))$, and the second model is given by $ G_\theta(p_{z_0^1}, \dots, p_{z_0^N}, p_{\alpha^1}, \dots, p_{\alpha^N }) = g_{1}(\sum_{k=1}^{N}g_{0}({z}_{0}^{k}) \odot {\alpha}^{k})$. The latent codes $z_0^k$ are i.i.d samples for $p_{z_0}$, and the channel importance $\alpha^k$ are sampled from $p_\alpha$. Specifically,  a vector $\alpha' \in \R^{N}$ is sampled from $p_{\alpha'} \sim \text{Dir}_N(1)$, where $\text{Dir}_N(1)$ is the flat Dirichlet distribution, i.e.\ the uniform distribution over the $(N-1)$-dimensional simplex. Then each vector $\alpha^k$ is taken to be $\alpha^k = \{\alpha'\}_k \cdot \bm{1}$ where $ \bm{1}$ is the vector of all ones and $ \{\alpha'\}_k$ is the $k$-th entry of the vector $\alpha'$. Note this leads to each channel being weighted equally during training. 


%Recall that the mGANprior Algorithm \ref{alg:mGAN} increases  the latent variables used to the input codes $\{z_0^k\}_{k=1}^N$ and the channel importance $\{\alpha^k\}_{k=1}^N$  (Figure \ref{fig:rtil_mgan} left and the discussion in Section \ref{sec:mGANpiror}). Applying, therefore, RTIL we are led to then train, via the min-max formulation \eqref{eq:min-max}, the family of generative networks with shared weights $G_\theta = \{G_{\theta}(\overbrace{p_{z_{0}}, \dots, p_{z_{0}}}^{N}, 0), G_{\theta}(\overbrace{p_{z_{0}}, \dots, p_{z_{0}}}^{N}, p_\alpha) \}$ where  $p_\alpha$ is a probability distribution over the channel importance $\{\alpha^k\}_{k=1}^N$ (Figure \ref{fig:rtil_mgan} right). 
%In particular, inspired by the role of the $\alpha$s as weight for the features maps outputs of $g_0$, a vector $\alpha' \in \R^{N}$ is sampled from $p_{\alpha'} \sim \text{Dir}_N(1)$, where $\text{Dir}_N(1)$ is the flat Dirichlet distribution, i.e.\ the uniform distribution over the $(N-1)$-dimensional simplex. Then each vector $\alpha^k$ is taken to be $\alpha^k = \{\alpha'\}_k \cdot \bm{1}$ where $ \bm{1}$ is the vector of all ones and $ \{\alpha'\}_k$ is the $k$-th entry of the vector $\alpha'$.
%This choice is made to control the scaling of the output of the layer $g_0$ and to not artificially  skew the channel importance during training, leaving those parameters to be solved for during optimization. 


%Applying our principle to the inversion method mGan prior will follow underline principle of RTIL by simultaneously training a vanilla model, and a second model that can map k many latent codes to image space. The models parameter share with each other. Our method can be extended to larger family of generative models, here is the two model example. The pipeline for training RTIL-mGAN closely follows figure \ref{fig:rtil_mgan}. During training a distribution is induced at an intermediate layer over k-dimensional simplex, sampling uniformly from a k-dimensional simplex is chosen to kept scaling of the output of the layers consistent. By selecting this distribution we are not putting an emphasis on channel importance, but leaving that parameter to be solved for during optimzation. 



==> sections/sec-theory.tex <==

\section{Theoretical Model for Compressed Sensing with RTIL}

In this section, we examine a simple theoretical model for compressive sensing with RTIL.  To provide the most easily understandable context, we consider the case of a generative model given by a two-layer linear neural network.  Further, we consider the case where the generative model is trained in a supervised manner, and we consider the regime of infinite training data. {The supervised setting allows us to avoid discussing the different methods for learning generative models,  and working in the infinite data regime we avoid statistical estimation errors}.

%{\color{red} more comments on why we assume these?} 

We assume that the true signal distribution is given by
$x = G^\star(z_0, z_1) = \Wstar_1( \Wstar_0 z_0 + z_1 )$, 
where 
$G^\star: \R^{n_0} \times \R^{n_1} \to \R^{n_d}$, $z_0 \sim \mathcal{N}(0,I_{n_0})$ and $z_1 \sim \mathcal{N}(0,I_{n_1})$ drawn independently, and 
  where $\Wstar_1 \in \R^{n_d \times n_1}$ and $\Wstar_0 \in \R^{n_1 \times n_0}$. We moreover assume that $n_0 < n_1 < n_d$, and $\Wstar_0, \Wstar_1$ are full rank.  We furthermore assume that $\Wstar_0$ is known but that $\Wstar_1$ is unknown.
 
\subsection{Training the Models}  
We consider the training of two generative models.  The first model is analogous to GAN training without RTIL.  In it, $\G^{0} (z_0) = W_1^{0}( \Wstar_0 z_0)$.  %Note that the model does not depend on $z_1$.    
The second model is analogous to GAN training with RTIL.  In it, $G^{1}(z_0, z_1) = W_1^{1}( \Wstar_0 z_0 + z_1)$. 

Training each model consists of estimating $W_1^{i}$ under a least squares loss.  As we consider the idealized regime of infinite training data, we obtain the following estimates:
%$G^{(i)}: \R^{n_0} \times \R^{n_1} \to \R^{n_d}$ for $i = 1, 2$. Model $G^{(1)}$ is trained without regularizing the intermediate layer, while model $G^{(2)}$ is trained with regularization (RTIL). 
%To simplify the discussion, we will assume that $\Wstar_0 \in \R^{n_1 \times n_0}$ is known, the models are trained in a supervised way and the infinite data regime is well approximated. Specifically, $G^{(1)}: (z_0, z_1) \mapsto W_{1}^{(1)}(\Wstar_0 z_0 + z_1 )$
%where 
%%\begin{equation}\label{eq:W11}
%%    W_1^{(1)} \in \argmin_{W_1 \in \R^{n_d \times n_1}} \E_{\substack{z_0 \sim \mathcal{N}(0,I_{n_0}) \\ z_1 \sim \mathcal{N}(0,I_{n_1})}} \| G^\star(z_0, z_1) - G^{(1)}(z_0, 0) \|_2^2
%%\end{equation}
\begin{equation}\label{eq:W11}
    W_1^{0} \in \argmin_{W_1 \in \R^{n_d \times n_1}} \E_{z_0, z_1} \| G^\star(z_0, z_1) - W_1 \Wstar_0 z_0 \|_2^2,
\end{equation}
and
%and $G^{(2)}: (z_0, z_1) \mapsto W_{1}^{(2)}(\Wstar_0 z_0 + z_1 )$ where 
\begin{equation}\label{eq:W12}
    W_1^{1} \in \argmin_{W_1 \in \R^{n_d \times n_1}} \E_{z_0, z_1} \| G^\star(z_0, z_1) - W_1(\Wstar_0 z_0 + z_1) \|_2^2.
\end{equation}
%Notice how in \eqref{eq:W11} the intermediate layer variable is not regularized during training, while it is regularized in \eqref{eq:W12}, which corresponds to RTIL in this simplified model.

The next lemma is a simple consequence of the property of the Gaussian distribution. 
\begin{lemma}\label{lemma:training} 
Let $W_1^{0}$ satisfy in \eqref{eq:W11} then $W_1^{0} \Wstar_0 = \Wstar_1 \Wstar_0$. 
Moreover, 
there exists a unique $W_1^{1}$ solution of \eqref{eq:W12}, given by $W_1^{1} = \Wstar_1$.
\end{lemma}
While the above lemma shows that $W_1^{0}$ will equal $\Wstar_1$ on the range of $\Wstar_0$, its behavior on the space orthogonal to the range of $\Wstar_0$ depends on how \eqref{eq:W11} is solved. To simplify the discussion below we will consider $W_1^{0}$ to be the minimum (Frobenius) norm solution of \eqref{eq:W11}. 
%For example, if \eqref{eq:W11} was solved by a gradient descent method, the restriction of $W_1^{(1)}$  on the space orthogonal to the range of $\Wstar_0$ would be fixed at initialization. 

\subsection{Compressed Sensing}
We next analyze the compressed sensing problem with the trained generative models.  Let $x^\star = G^\star(z_0^\star, z_1^\star)$ be an unknown signal, where $z_0^\star \sim \mathcal{N}(0,I_{n_0})$ and $z^\star_1 \sim \mathcal{N}(0,I_{n_1})$. We consider the problem of recovering $x^\star$ given compressed linear measurements $y = A x^\star \in \R^{m}$ where $n_1~\leq~m~<~n_d$.  For $i = 1, 2$, we let
\begin{equation*}
\begin{aligned}
    z_0^{(i)} &= \argmin_{z_0 \in \R^{n_0}} \| y - A G^{i}(z_0, 0) \|_2^2, \\
    z_1^{(i)} &= \argmin_{z_1 \in \R^{n_1}} \| y - A G^{i}(z_0^{(i)}, z_1)\|_2^2. \\
\end{aligned} 
\end{equation*}
Here, with a slight abuse of notation we denote by $G^{0}$ the model trained with \eqref{eq:W11} and where $z_1$ is introduced as an intermediate variable. In it, $G^{0}(z_0, z_1) = W_1^{0}( \Wstar_0 z_0 + z_1)$.
Moreover, we take $z_1^{(0)}$ to be the minimum norm solution. As shown in the proof $z_0^{(0)}$ and $(z_0^{(1)}, z_1^{(1)})$ are unique.
Notice that $(z_0^{(0)}, z_1^{(0)})$ and $(z_0^{(1)}, z_1^{(1)})$ correspond to the latent vector and intermediate layer variables obtained applying the ILO Algorithm \ref{alg:ILO} with inputs  $\{G^{0}, A, y \}$ and $\{G^{1}, A, y \}$ respectively. 

The following lemma quantifies the reconstruction errors made by using the two generative models. 

\begin{lemma}\label{lemma:CS}
Assume that $\Wstar_0, \Wstar_1$ are full rank. Let $W^{0}_1$ be the minimum norm solution of \eqref{eq:W11} and $W^{1}_1$ be the solution of \eqref{eq:W12}. Let $A \in \R^{m \times n_d}$ with i.i.d. $\mathcal{N}(0,1)$ entries. Then with probability $1$
\begin{multline}\label{eq:ERR1}
    \E_{z^\star_0, z^\star_1} \big[\| G^\star(z^\star_0, z^\star_1) -  G^{0}(z_0^{(0)}, z_1^{(0)}) \|^2 \big] \\ \geq \max_{h \in \text{range}(\Wstar_0)^\perp}\|(I_{n_d} - \mathcal{P}_{\Wstar_1 \Wstar_0} \big) \Wstar_1 h\|_2^2 > 0 
\end{multline}
and 
\begin{equation}\label{eq:ERR2}
    \E_{z^\star_0, z^\star_1} [\| G^\star(z^\star_0, z^\star_1) -  G^{1}(z_0^{(1)}, z_1^{(1)}) \|^2] =0.
\end{equation}
%where  $ \mathcal{P}_{W^{(1)}_1}$ is the orthogonal projector onto the range of $W^{(1)}_1$.
\end{lemma}
The above results illustrate why training generative models using RTIL can enable better compressed sensing performance.  In the simplified setting of a two-layer linear neural network trained in a supervised manner with a known first layer and in the infinite data regime, we see that the lower dimensional generative model incurs error in the second layer's weights in the orthogonal complement of the range of the first layer.  This results in an increase in the reconstruction error when solving compressed sensing.

%{\color{red}MAYBE REMOVE} the effects of regularizing during training the intermediate layers variables of a generative model used for inverse problems. In particular, demonstrating that a model trained without intermediate variable regularization leads to larger reconstruction when solving compressed sensing, compared to a model trained with regularization. 

%{\color{red}MAYBE REMOVE} The effects of the regularized training is to regularize the behavior of the second layer $W_1$ in the directions orthogonal to the range of the first layer. These directions are not regularized by the standard training methods, but are used during inversion. 



